A Unified Maximum Likelihood Approach for Optimal Distribution Property Estimation

The advent of data science has spurred interest in estimating properties of distributions over large alphabets. Fundamental symmetric properties such as support size, support coverage, entropy, and proximity to uniformity, received most attention, with each property estimated using a different technique and often intricate analysis tools. We prove that for all these properties, a single, simple, plug-in estimator---profile maximum likelihood (PML)---performs as well as the best specialized techniques. This raises the possibility that PML may optimally estimate many other symmetric properties.

==> glodef.tex <==
% Theorem-like environments

\makeatletter
\@ifundefined{theorem}{% Theorems (each with its own style)
  \theoremstyle{definition}
  \newtheorem{definition}{Definition}
  \theoremstyle{plain}
  \newtheorem{theorem}{Theorem}
  \newtheorem{corollary}{Corollary}
  \newtheorem{lemma}{Lemma}
  \newtheorem{claim}{Claim}
  \newtheorem{fact}{Fact}
  \newtheorem*{unnumberedfact}{Fact}
  \theoremstyle{remark}
  \newtheorem{remark}{Remark}
  \newtheorem{question}{Question}
  \newtheorem*{notation}{Notation}
  \newtheorem{example}{Example}
  \newtheorem{observation}{Observation}
}{}
\makeatother
\newenvironment{proofof}[1]{\noindent{\bf Proof of {#1}:~~}}{\(\qed\)}

% Begin / End Theorems

\def \bthm#1{\begin{#1}\upshape\quad}
\def \ethm#1{\rqed\end{#1}}
\def \ethmp#1{\end{#1}}     % No box, when ends in displayed equation

\def \bClaim     {\bthm{Claim}}
\def \eClaim     {\ethm{Claim}}
\def \eClaimp    {\ethmp{Claim}}
\def \bConjecture {\bthm{Conjecture}}
\def \eConjecture {\ethm{Conjecture}}
\def \eConjecturep{\ethmp{Conjecture}}
\def \bCorollary {\bthm{Corollary}}
\def \eCorollary {\ethm{Corollary}}
\def \eCorollaryp{\ethmp{Corollary}}
\def \bCounter   {\bthm{CounterExample*}}
\def \eCounter   {\ethm{CounterExample*}}
\def \eCounterp  {\ethmp{CounterExample}}
\def \bDefinition{\bthm{Definition}}
\def \eDefinition{\ethm{Definition}}
\def \eDefinitionp{\ethmp{Definition}}
\def \bExample   {\bthm{Example}}
\def \eExample   {\ethm{Example}}
\def \eExamplep  {\ethmp{Example}}
\def \bExercise  {\bthm{Exercise}}
\def \eExercise  {\ethm{Exercise}}
\def \eExercisep {\ethmp{Exercise}}
\def \bIntuition {\bthm{Intuition}}
\def \eIntuition {\ethmp{Intuition}}
\def \bJoke      {\bthm{Joke}}
\def \eJoke      {\ethm{Joke}}
\def \bLemma     {\bthm{Lemma}}
\def \eLemma     {\ethm{Lemma}}
\def \eLemmap    {\ethmp{Lemma}}
\def \bOpen      {\bthm{Open problem}}
\def \eOpen      {\ethm{Open problem}}
\def \eOpenp     {\ethmp{Open problem}}
\def \bProperty  {\bthm{Property}}
\def \eProperty  {\ethm{Property}}
\def \ePropertyp {\ethmp{Property}}
\def \bQuestion  {\bthm{Question}}
\def \eQuestion  {\ethm{Question}}
%\def \bRemark    {\bthm{Remark}}
%\def \eRemark    {\ethm{Remark}}
\def \bResult    {\bthm{Result}}
\def \eResult    {\ethm{Result}}
\def \bTheorem   {\bthm{Theorem}}
\def \eTheorem   {\ethm{Theorem}}
\def \eTheoremp  {\ethmp{Theorem}}

\def \bSubexa    {\begin{subexa}}
\def \eSubexa    {\ethm{subexa}}
\def \eSubexap   {\ethmp{subexa}}

% Environments

\newenvironment{Problem}{\textbf{Problem}\\ \begin{enumerate}}{\end{enumerate}}
\newenvironment{Problems}{\textbf{Problems}\\ \begin{enumerate}}{\end{enumerate}}

%\newenvironment{Problems}{\begin{trivlist}\item[]{\textbf{Problems}}{\end{trivlist}}}

% Headers

\def \skpbld#1{\par\noindent\textbf{#1}\quad}
\def \skpblds#1{\skpbld{#1}\par\noindent}

\def \Answer   {\skpbld{Answer}}
\def \Answers  {\skpblds{Answers}}
\def \Basis    {\skpbld{Basis}}
\def \Check    {\skpbld{Check}}
%\def \Example  {\skpbld{Example}}
\def \Examples {\skpbld{Examples}}
\def \Intuition{\skpbld{Intuition}}
\def \Method   {\skpbld{Method}}
\def \Methods  {\skpblds{Methods}}
\def \Outline  {\skpbld{Outline}}
\def \Proof    {\skpbld{Proof}}
\def \Proofs   {\skpblds{Proofs}}
%\def \Problem  {\skpbld{Problem}}
%\def \Problems {\skpblds{Problems}}
\def \Proline  {\skpbld{Proof Outline}}
%\def \Remark   {\skpbld{Remark}}
\def \Remarks  {\skpblds{Remarks}}
\def \Solution {\skpbld{Solution}}
\def \Solutions{\skpblds{Solutions}}
\def \Verify   {\skpbld{Verify}}
\def \Step     {\skpbld{Step}}

% Ignores

\newcommand{\ignore}[1]{}

% Problems & solutions

\newcommand{\problem}[1]{#1}
\newcommand{\solution}[1]{{\\ \bf Solution}\quad #1}
%\newcommand{\solution}[1]{\mbox{}\\ \medskip\noindent{\bf Solution\medskip}#1}
%\newcommand{\solution}[1]{}

\newcommand{\source}[1]{(Taken from~\cite{#1})}
%\newcommand{\source}[1]{}

\newcommand{\modifiedfrom}[1]{(Modified from~\cite{#1})}
%\newcommand{\modifiedfrom}[1]{}

\newcommand{\takenfrom}[1]{(Taken from~\cite{#1})}
%\newcommand{\takenfrom}[1]{}

\newcommand{\reportedby}[1]{Reported by #1.}
%\newcommand{\reportedby}[1]{}

\newcommand{\hint}[1]{Hint: #1}
%\newcommand{\hint}[1]{}

\newcommand{\joke}[1]{\footnote{#1}}
\newcommand{\trivia}[1]{\footnote{#1}}

% Equation formatting

\newcommand{\spreqn}[1]{{\qquad\text{#1}\qquad}}

% Blackboard fonts
\newcommand{\II}{\mathbb{I}} % Added by Theertha on April 16th 2013.
\newcommand{\EE}{\mathbb{E}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\PP}{\mathbb{P}}

% probability
\newcommand{\expectation}[1]{\EE\left[#1\right]}

% Number sets

\newcommand{\complex}{\CC}
\newcommand{\integers}{\ZZ}
\newcommand{\naturals}{\NN}
\newcommand{\positives}{\PP}
\newcommand{\rationals}{\QQ}
\newcommand{\reals}{\RR}

\newcommand{\realsge}{{\reals_{\ge}}}
\newcommand{\realsp}{\reals^+}
\newcommand{\integersp}{\integers^+}
\newcommand{\integerss}[1]{\integers_{\ge{#1}}}

% boldface

\def \ba     {{\bf a}}
\def \bx     {{\bf x}}
\def \by     {{\bf y}}

\def \bA     {{\bf A}}
\def \bB     {{\bf B}}
\def \bC     {{\bf C}}
\def \bD     {{\bf D}}
\def \bF     {{\bf F}}
\def \bG     {{\bf G}}
\def \bL     {{\bf L}}
\def \bQ     {{\bf Q}}
\def \bR     {{\bf R}}
\def \bS     {{\bf S}}
\def \bT     {{\bf T}}
\def \bX     {{\bf X}}
\def \bY     {{\bf Y}}
\def \bZ     {{\bf Z}}

% caligraphics

\def \cA     {{\cal A}}
\def \cB     {{\cal B}}
\def \cC     {{\cal C}}
\def \cD     {{\cal D}}
\def \cE     {{\cal E}}
\def \cF     {{\cal F}}
\def \cG     {{\cal G}}
\def \cH     {{\cal H}}
\def \cI     {{\cal I}}
\def \cK     {{\cal K}}
\def \cL     {{\cal L}}
\def \cM     {{\cal M}}
\def \cN     {{\cal N}}
\def \cO     {{\cal O}}
\def \cP     {{\cal P}}
\def \cQ     {{\cal Q}}
\def \cR     {{\cal R}}
\def \cS     {{\cal S}}
\def \cT     {{\cal T}}
\def \cU     {{\cal U}}
\def \cV     {{\cal V}}
\def \cW     {{\cal W}}
\def \cX     {{\cal X}}
\def \cY     {{\cal Y}}
\def \cZ     {{\cal Z}}

% vectors

\def \vct#1{{\overline{#1}}}

\def \vcta  {{\vct a}}
\def \vctb  {{\vct b}}
\def \vctq  {{\vct q}}
\def \vcts  {{\vct s}}
\def \vctu  {{\vct u}}
\def \vctv  {{\vct v}}
\def \vctx  {{\vct x}}
\def \vcty  {{\vct y}}
\def \vctz  {{\vct z}}
\def \vctp  {{\vct p}}

\def \vctV  {{\vct V}}
\def \vctX  {{\vct X}}
\def \vctY  {{\vct Y}}
\def \vctZ  {{\vct Z}}

\def \vctbeta  {{\vct\beta}}

% Random variables

\newcommand{\rnd}[1]{{\boldsymbol #1}}

\newcommand{\rndd}{{\rnd d}}
\newcommand{\rndl}{{\rnd l}}
\newcommand{\rndp}{{\rnd p}}
\newcommand{\rnds}{{\rnd s}}
\newcommand{\rndx}{{\rnd x}}
\newcommand{\rndy}{{\rnd y}}
\newcommand{\rndz}{{\rnd z}}

%\newcommand{\poi}{{\rm poi}}
\newcommand{\Var}{{\rm Var}}

% following should not exist (indicate random sets)

\newcommand{\rndR}{{\rnd R}}
\newcommand{\rndT}{{\rnd T}}

% arrow vectors

\newcommand{\rvc}{{\overrightarrow c}}

% Abbreviations - \xspace puts space iff there is space after command

\newcommand{\eg}{\textit{e.g.,}\xspace}
\newcommand{\ie}{\textit{i.e.,}\xspace}  % note that overridden in spanish
%\newcommand{\iid}{\textit{i.i.d.}\xspace} 
\newcommand{\iid}{\textit{i.i.d.}} % Edit by Theertha, \xspace not compiling

\newcommand{\etc}{etc.\@\xspace}

% Colors

%\definecolor{light}{gray}{.75}


% marginal notes

\newcommand{\mrgs}[2]{\# #1 \#{\marginpar{#2}}}

\newcommand{\mrgcgd}[1]{\mrgs{#1}{CHANGED}}
\newcommand{\mrgchk}[1]{\mrgs{#1}{CHECK}}
\newcommand{\mrgfix}[1]{\mrgs{#1}{FIX}}
\newcommand{\mrgnew}[1]{\mrgs{#1}{NEW}}

% qed's --  Also consider \qedhere

\def \eqed    {\eqno{\qed}}
\def \rqed    {\hbox{}~\hfill~$\qed$}

% sequences

\def \upto  {{,}\ldots{,}}

\def \zn    {0\upto n}
\def \znmo  {0\upto n-1}
\def \znpo  {0\upto n+1}
\def \ztnmo {0\upto 2^n-1}
\def \ok    {1\upto k}
\def \on    {1\upto n}
\def \onmo  {1\upto n-1}
\def \onpo  {1\upto n+1}

% sets

\def \sets#1{{\{#1\}}}
\def \Sets#1{{\left\{#1\right\}}}

\def \set#1#2{{\sets{{#1}\upto{#2}}}}

\def \setpmo   {\sets{\pm 1}}
\def \setmpo   {\{-1{,}1\}}
\def \setzo    {\{0{,}1\}}
\def \setzn    {\{\zn\}}
\def \setznmo  {\{\znmo\}}
\def \setztnmo {\{\ztnmo\}}
\def \setok    {\{\ok\}}
\def \seton    {\{\on\}}
\def \setonmo  {\{\onmo\}}
\def \setzon   {\setzo^n}
\def \setzos   {\setzo^*}

\def \inseg#1{{[#1]}} % use \intsgm instead
\newcommand{\intsgm}[1]{{[#1]}}

% functions

\def \ord    {\#}

\def \suml   {\sum\limits}
\def \prodl  {\prod\limits}

% Set operations


%\DeclareMathOperator*{\union}{\cup}  %Commented by Theertha on April 15
%\DeclareMathOperator*{\Union}{\bigcup}  %Commented by Theertha on April 15

\newcommand{\unionl}{\union\limits}
\newcommand{\Unionl}{\Union\limits}
 
%\DeclareMathOperator*{\inter}{\cap}  %Commented by Theertha on April 15
%\DeclareMathOperator*{\Inter}{\bigcap}   %Commented by Theertha on April 15

\newcommand{\interl}{\inter\limits}
\newcommand{\Interl}{\Inter\limits}

% Floors, Ceilings, Absolute value

\def \ceil#1{{\lceil{#1}\rceil}}
\def \Ceil#1{{\left\lceil{#1}\right\rceil}}
\def \floor#1{{\lfloor{#1}\rfloor}}
\def \Floor#1{{\left\lfloor{#1}\right\rfloor}}
\def \absvlu#1{{|#1|}}
\def \Absvlu#1{{\left|{#1}\right|}}
\newcommand{\absv}[1]{\left|#1\right|}
% Parentheses, brackets

\def \paren#1{{({#1})}}
\def \Paren#1{{\left({#1}\right)}}
\def \brack#1{{[{#1}]}}
\def \Brack#1{{\left[{#1}\right]}}

%\def \frac#1#2{{{#1}\over{#2}}}
\def \frc#1#2{{\frac{#1}{#2}}}

\def \binomial#1#2{{{#1}\choose{#2}}}

\def \gcd#1#2{{{\rm gcd}\paren{{#1},{#2}}}}
\def \Gcd#1#2{{{\rm gcd}\Paren{{#1},{#2}}}}

\def \lcm#1#2{{{\rm lcm}\paren{{#1},{#2}}}}
\def \Lcm#1#2{{{\rm lcm}\Paren{{#1},{#2}}}}

% number theory

\newcommand{\base}[2]{{[#1]_{#2}}}

% equalities

\newcommand{\ed}{\stackrel{\text{def}}{=}}
\newcommand{\eqdef}{{:=}}

\newcommand{\cnvprb}{\stackrel{\mathrm{p}}{\to}}
\newcommand{\cnvdst}{\stackrel{\mathrm{d}}{\to}}
\newcommand{\cnvas}{\stackrel{\mathrm{a.s.}}{\to}}

\def \gap    {\ \hbox{\raisebox{-.6ex}{$\stackrel{\textstyle>}{\sim}$}}\ }

\newcommand{\al}[1]{\stackrel{\mathit{{#1}}}{<}}
\newcommand{\ag}[1]{\stackrel{\mathit{{#1}}}{>}}
\newcommand{\ale}[1]{\stackrel{\mathit{{#1}}}{\le}}
\newcommand{\age}[1]{\stackrel{\mathit{{#1}}}{\ge}}
\newcommand{\aeq}[1]{\stackrel{\mathit{{#1}}}{=}}

%\newcommand{\eae}{\approx} % exponentially asymptotically eq - replace by \ere
%\newcommand{\eal}{\stackrel<\approx} % replace by \erl

\newcommand{\re}{\sim}
\newcommand{\rle}{\stackrel<\sim} % roughly (asymptotically taken) <=
%\newcommand{\rl}{\stackrel<\sim}
\newcommand{\rge}{\stackrel>\sim}
%\newcommand{\rg}{\stackrel>\sim}

\newcommand{\ere}{\approx} % exponentially roughly equal
\newcommand{\erle}{\stackrel<\approx}
%\newcommand{\erl}{\stackrel<\approx}
\newcommand{\erge}{\stackrel>\approx}
%\newcommand{\erg}{\stackrel>\approx}

% Relations

\newcommand{\independent}{\perp\!\!\!\perp}

% values

\def \half    {{\frac12}}
\def \quarter {{\frac14}}
\def \oo#1{{\frac1{#1}}}

% probability

\newcommand{\pr}{{p}} % phase out in favor of \prb
\newcommand{\prb}{{p}} 

\newcommand{\prbs}[1]{{\prb^{(#1)}}}

\newcommand{\Prb}{\text{Pr}}
%\newcommand{\Pr}{{\text{Pr}}} % phase out in favor of \Prb
\newcommand{\Prn}{\text{Pr}}  % phase out in favor of \Prb

\newcommand{\Prs}[1]{\Pr\Paren{#1}} % phase out in favor of \Prbs
\newcommand{\Prbs}[1]{{\Prb^{(#1)}}} % Check if used - phase out
\newcommand{\probof}[1]{\Pr\Paren{#1}}

% notation

\def \iff    {{\it iff }}
\def \th     {{\rm th }}

% ignore

\def\ignore#1{}

% Logic

\newcommand{\ra}{\rightarrow}
\def \contra {{\leftrightarrows}}
\newcommand{\ol}[1]{{\overline{#1}}}
%\def \ob {\overline}

\def \ve {{\lor}} % needed?
\def \eq {{\equiv}} % needed?

% spaces

\newcommand{\spcin}{\hspace{1.0in}}
\newcommand{\spchin}{\hspace{.5in}}

% Default text appears in regular print in both book and class versions. 
% There are two types of text that need to be highlighted in class:
% clson - not mentioned in book version (eg jokes)
% clsbk - regular text in book (the parts that need be said)

%For book:
%\newcommand{\clson}[1]{}
%\newcommand{\clsbk}[1]{#1}
%For class:
\newcommand{\clson}[1]{\colorbox{light}{{#1}}}
\newcommand{\clsbk}[1]{\colorbox{light}{{#1}}}

%\newcommand{\bi}{\begin{aopl}}
%\newcommand{\ei}{\end{aopl}}

\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
%\newcommand{\bq}{\begin{quote}}
%\newcommand{\eq}{\end{quote}}

\newenvironment{aopl}
  {\begin{list}{}{\setlength{\itemsep}{4pt plus 2pt minus 2pt}}}
  {\end{list}}

% operators

\newcommand{\flnpwr}[2]{{#1^{\underline{#2}}}} % Falling power

\def\orpro{\mathop{\mathchoice
   {\vee\kern-.49em\raise.7ex\hbox{$\cdot$}\kern.4em}
   {\vee\kern-.45em\raise.63ex\hbox{$\cdot$}\kern.2em}
   {\vee\kern-.4em\raise.3ex\hbox{$\cdot$}\kern.1em}
   {\vee\kern-.35em\raise2.2ex\hbox{$\cdot$}\kern.1em}}\limits}

\def\andpro{\mathop{\mathchoice
 {\wedge\kern-.46em\lower.69ex\hbox{$\cdot$}\kern.3em}
 {\wedge\kern-.46em\lower.58ex\hbox{$\cdot$}\kern.25em}
 {\wedge\kern-.38em\lower.5ex\hbox{$\cdot$}\kern.1em}
 {\wedge\kern-.3em\lower.5ex\hbox{$\cdot$}\kern.1em}}\limits}

\def\inter{\mathop{\mathchoice
   {\cap}
   {\cap}
   {\cap}
   {\cap}}}
\def\interl {\inter\limits}

\def\carpro{\mathop{\mathchoice
   {\times}
   {\times}
   {\times}
   {\times}}\limits}

\def\simge{\mathrel{%
   \rlap{\raise 0.511ex \hbox{$>$}}{\lower 0.511ex \hbox{$\sim$}}}}

\def\simle{\mathrel{
   \rlap{\raise 0.511ex \hbox{$<$}}{\lower 0.511ex \hbox{$\sim$}}}}

\newcommand{\pfx}{{\prec}}
\newcommand{\pfxeq}{{\preceq}}

\newcommand{\sfx}{{\succ}}
\newcommand{\sfxeq}{{\succeq}}

% for old documents

\newcommand{\twlrm}{\fontsize{12}{14pt}\normalfont\rmfamily}
\newcommand{\tenrm}{\fontsize{10}{12pt}\normalfont\rmfamily}

% picture macros

\newcommand{\grid}[2]{				% grid{width}{height}
  \multiput(0,0)(1,0){#1}{\line(0,1){#2}}
  \put(#1,0){\line(0,1){#2}}
  \multiput(0,0)(0,1){#2}{\line(1,0){#1}}
  \put(0,#2){\line(1,0){#1}}
}

% inductiion macros

%\newcommand{\induction}[3]{
%Inductive statement: {#1}\\
%We prove: {#2}\\
%Basis: {#3}\\
%Step: {#4}\\
%Proof of step: {#5}
%}


\newcommand{\Sparen}[1]{\left[#1\right]}
\newcommand{\Order}{O}
\newcommand{\order}{o}






